Private and Resource-Bounded Locally Decodable Codes for Insertions and Deletions

We construct locally decodable codes (LDCs) to correct insertion-deletion errors in the setting where the sender and receiver share a secret key or where the channel is resource-bounded. Our constructions rely on a so-called "Hamming-to-InsDel" compiler (Ostrovsky and Paskin-Cherniavsky, ITS '15 & Block et al., FSTTCS '20), which compiles any locally decodable Hamming code into a locally decodable code resilient to insertion-deletion (InsDel) errors. While the compilers were designed for the classical coding setting, we show that the compilers still work in a secret key or resource-bounded setting. Applying our results to the private key Hamming LDC of Ostrovsky, Pandey, and Sahai (ICALP '07), we obtain a private key InsDel LDC with constant rate and polylogarithmic locality. Applying our results to the construction of Blocki, Kulkarni, and Zhou (ITC '20), we obtain similar results for resource-bounded channels; i.e., a channel where computation is constrained by resources such as space or time.

==> fig-ldc-game.tex <==
\begin{figure}[tp]
	\begin{boxedalgo}
		$\LDCgame[\cA,x,\rho,p]\colon$
		\begin{enumerate}
%			\setcounter{enumi}{-1}
%			\item If $C$ is a private code, the challenger generates secret key $\sk \gets \Gen(1^\lambda)$ and computes a codeword $y \gets \Enc(x,\sk)$ for message $x\in \Sigma^k$ and sends $y$ to $\cA$.
			\item Otherwise challenger computes a codeword $y \gets \Enc(x)$ for message $x \in \Sigma^k$, and sends $y$ to $\cA$.
			
			\item The attacker outputs a corrupted codeword $y' \gets \cA(x,y,\rho,p,k,K,\lambda)$, where $y' \in \Sigma^*$.
			
			\item The output of the experiment is determined as follows:
		\end{enumerate}
		\begin{align*}
			&\LDCgame[\cA,x,\rho,p]\\
			&= \begin{cases}
				1 & \text{if } \dist(y,y') \leq \rho \text{ and }\\
				& \exists i \in [k] \colon \Pr[\Dec^{y'}(i) = x_i] < p \\
				0 & \text{otherwise}
			\end{cases}
		\end{align*}
		We say that $\cA$ wins the experiment if the output is $1$; otherwise we say that $\cA$ loses the experiment.
	\end{boxedalgo}
	\caption{Security game defining the interaction between an attacker and an honest party for code $C[K,k,q_1,q_2] = (\Enc,\Dec)$,}\label{fig:ldc-game}
\end{figure}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

==> fig-priv-ldc-game.tex <==


\begin{figure}[tp]
\begin{boxedalgo}
	$\privLDCgame[\cA,x,\lambda,\rho,p]\colon$
	\begin{enumerate}
		\item The challenger generates a secret key $\sk \gets \Gen(1^\lambda)$, computes a codeword $y \gets \Enc(x,\sk)$ for message $x \in \Sigma^k$, and sends codeword $y$ to $\cA$.
		
		\item The attacker outputs a corrupted codeword $y' \gets \cA(x,y,\lambda,\rho,p,k,K)$, where $y' \in \Sigma^*$.
		
		\item The output of the experiment is determined as follows:
	\end{enumerate}
	\begin{align*}
		&\privLDCgame[\cA,x,\lambda,\rho,p]\\
		&= \begin{cases}
			1 & \text{if } \dist(y,y') \leq \rho \text{ and }\\
			& \exists i \in [k] \colon \Pr[\Dec^{y'}(i,\sk) = x_i] < p \\
			0 & \text{otherwise}
		\end{cases}
	\end{align*}
	We say that $\cA$ wins the experiment if the output is $1$; otherwise we say that $\cA$ loses the experiment.
\end{boxedalgo}
\caption{Security game defining the interaction between an attacker and an honest party for code $C[K,k,q_1,q_2,\lambda] = (\Gen,\Enc,\Dec)$.\label{fig:priv-ldc-game}}
%Note that $\cA$ is not given secret key $\sk$.}
\end{figure}






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
